Polynomial Preconditioning for Gradient Methods

We study first-order methods with preconditioning for solving structured nonlinear convex optimization problems. We propose a new family of preconditioners generated by symmetric polynomials. They provide first-order optimization methods with a provable improvement of the condition number, cutting the gaps between highest eigenvalues, without explicit knowledge of the actual spectrum. We give a stochastic interpretation of this preconditioning in terms of coordinate volume sampling and compare it with other classical approaches, including the Chebyshev polynomials. We show how to incorporate a polynomial preconditioning into the Gradient and Fast Gradient Methods and establish the corresponding global complexity bounds. Finally, we propose a simple adaptive search procedure that automatically chooses the best possible polynomial preconditioning for the Gradient Method, minimizing the objective along a low-dimensional Krylov subspace. Numerical experiments confirm the efficiency of our preconditioning strategies for solving various machine learning problems.

==> Introduction/Contents.tex <==
\subsection{Contents}

  \textbf{TODO: merge with contributions}

The rest of the paper is organized as follows.
In Section~\ref{SectionNotation},
we formulate our optimization problem of interest in the composite form,
our main assumptions, and notation which is used within the rest of the paper.
We also provide several examples that satisfy our assumptions
and which highlight our motivation.
Section~\ref{SectionGM} is devoted to the
preconditioned first-order
optimization algorithms that we use for solving our problem.
We study the convergence of the basic Gradient Method
and the accelerated Fast Gradient Method with a general
(arbitrarily fixed) preconditioning matrix.
In Section~\ref{SectionSymmetric},
we present a new family of Symmetric Polynomial Preconditioners.
We list their main properties
and show how they can be incorporated into the first-order optimization schemes.
In Section~\ref{SectionKrylov}, we study a general class
of polynomial preconditioners and review some of the classical approaches,
including cutting off the eigenvalues and the Chebyshev polynomials.
We show how these techniques are related to our new family.
Then, we propose an adaptive procedure based on the Krylov subspace minimization
that achieves the best possible preconditioning guarantee.
Section~\ref{SectionExperiments} contains numerical experiments.
Missing proofs are provided in
the supplementary material.


==> KrylovSubspacePreconditioning/CuttingEigenvalues.tex <==



%\subsection{Cutting the Eigenvalues}
%\label{SubsectionCutting}
%\paragraph{Cutting the Eigenvalues.}

Let us assume that the top $\tau > 0$ eigenvalues of $\mat{B}$
are all \textit{separated}. Then, we can easily cut them off with the following
simple construction.
Define
\beq \label{QDef}
\ba{rcl}
q_{\tau}(s) & \Def &
\bigl( 1 - \frac{s}{\lambda_1} \bigr)
\bigl( 1 - \frac{s}{\lambda_2} \bigr)
\cdot \ldots \cdot
\bigl( 1 - \frac{s}{\lambda_{\tau}} \bigr).
\ea
\eeq


\begin{proposition} \label{PropositionCuttingEigenvalues}
  For any $\tau$, taking
  $
  \mat{P}  =  p_{\tau}(\mat{B}),
  $
  where $p_{\tau}(s) := \frac{1 + q_{\tau}(s) \cdot (\alpha s - 1)}{s}$
  with $q_{\tau}$ defined by \eqref{QDef} and $\alpha = \frac{2}{\lambda_{\tau + 1} + \lambda_n}$,
  the condition number is bounded by
  %\vspace{-2mm}
  %\beq \label{CuttingCondNumber}
  %\ba{rcl}
  $
  \frac{\beta}{\alpha}  \leq 
  \frac{\lambda_{\tau + 1}}{\lambda_n}.
  $
  %\ea
  %\eeq
\end{proposition}

